The Journey to Trustworthy AI: Pursuit of Pragmatic Frameworks

This paper reviews Trustworthy Artificial Intelligence (TAI) and its various definitions. Considering the principles respected in any society, TAI is often characterized by a few attributes, some of which have led to confusion in regulatory or engineering contexts. We argue against using terms such as Responsible or Ethical AI as substitutes for TAI. And to help clarify any confusion, we suggest leaving them behind. Given the subjectivity and complexity inherent in TAI, developing a universal framework is deemed infeasible. Instead, we advocate for approaches centered on addressing key attributes and properties such as fairness, bias, risk, security, explainability, and reliability. We examine the ongoing regulatory landscape, with a focus on initiatives in the EU, China, and the USA. We recognize that differences in AI regulations based on geopolitical and geographical reasons pose an additional challenge for multinational companies. We identify risk as a core factor in AI regulation and TAI. For example, as outlined in the EU-AI Act, organizations must gauge the risk level of their AI products to act accordingly (or risk hefty fines). We compare modalities of TAI implementation and how multiple cross-functional teams are engaged in the overall process. Thus, a brute force approach for enacting TAI renders its efficiency and agility, moot. To address this, we introduce our framework Set-Formalize-Measure-Act (SFMA). Our solution highlights the importance of transforming TAI-aware metrics, drivers of TAI, stakeholders, and business/legal requirements into actual benchmarks or tests. Finally, over-regulation driven by panic of powerful AI models can, in fact, harm TAI too. Based on GitHub user-activity data, in 2023, AI open-source projects rose to top projects by contributor account. Enabling innovation in TAI hinges on the independent contributions of the open-source community.

==> Tables/CollectingTrainingDataRiskMatrix.tex <==
\begin{table}[htbp]
    \centering
    % \begin{tabular}{|c|c|}
    \begin{tabularx}{\textwidth}{|X|X|}
        \hline
        \multirow{2}{*}{\textbf{Known Data Quality}} & \textbf{\KK} \\
        & Collecting biased or incomplete data. Mitigation: Diversify sources. \\
        \hline
        \textbf{\KU} & Collecting somewhat inaccurate data. Mitigation: Apply quality control measures. \\
        \hline
    \end{tabularx}
    \quad
    \begin{tabularx}{\textwidth}{|X|X|}
        \hline
        \multirow{2}{*}{\textbf{Unknown Data Quality}} & \textbf{\UK} \\
        & Collecting highly sensitive data. Mitigation: Implement strong security measures. \\
        \hline
        \textbf{\UU} & Collecting data without proper documentation. Mitigation: Investigate source, conduct analysis. \\
        \hline
    \end{tabularx}
\end{table}

\begin{itemize}
    \item \textbf{\KK:} Collecting user activity data-- training data-- from a biased source, such as a social media platform where users are more likely to express extreme views.
    \item \textbf{\KU:} Collecting training data that is not perfectly accurate, but is still sufficient for building an AI model.
    \item \textbf{\UK:} Collecting training data that is highly sensitive and if not handled by experienced data scientists, could result in discrimination against certain groups of people.
    \item \textbf{\UU:} Collecting training data that does not include its meta-data or proper documentation on its original source.
\end{itemize}



==> Tables/TableDefinitionsofTrust.tex <==
\begin{table}[h]
\centering
\caption{Definitions of Trust across Various Disciplines. (List from \citet{cho2015survey})}
\label{tab:trust_definitions}
\begin{tabular}{|p{0.2\textwidth}|p{0.6\textwidth}|p{0.2\textwidth}|}
\hline
\rowcolor{gray!30}        
\textbf{Discipline} & \textbf{Meaning of Trust} & \textbf{Source} \\
\hline
Philosophy & Risky action deriving from personal, moral relationships between two entities & Lahno [1999], James [2002], Rotter [1980] \\
\hline
Economics & Expectation upon a risky action under uncertainty and ignorance based on the calculated incentives for the action & Mayer et al. [1995], Kydd [2005] \\
\hline
Psychology & Cognitive learning process obtained from social experiences based on the consequences of trusting behaviors & Rotter [1980] \\
\hline
Organizational Management & Willingness to take risk and being vulnerable to the relationship based on ability, integrity, and benevolence & Mayer et al. [1995] \\
\hline
International Relations & Belief that the other party is trustworthy with the willingness to reciprocate cooperation & Kydd [2005] \\
\hline
Sociology & Subjective probability that another party will perform an action that will not hurt my interest under uncertainty and ignorance & Gambetta [1988] \\
\hline
Automation & Attitude that one agent will achieve another agent's goal in a situation where imperfect knowledge is given with uncertainty and vulnerability & Lee et al. [2006] \\
\hline
Computing \& Networking & Estimated subjective probability that an entity exhibits reliable behavior for particular operation(s) under a situation with potential risks & Cho et al. [2011] \\
\hline
\end{tabular}
\end{table}

